Prospects for a survey of the Galactic plane with the Cherenkov Telescope Array

Approximately one hundred sources of very-high-energy (VHE) gamma rays are known in the Milky Way. A survey of the entire Galactic Plane in the energy range from a few tens of GeV to a few hundred TeV has been proposed as a Key Science Project for the upcoming Cherenkov Telescope Array Observatory (CTAO). This article presents the status of the studies towards the Galactic Plane Survey (GPS). We build and make publicly available a sky model that combines data from observations of known gamma-ray emitters with state-of-the-art physically-driven models of synthetic populations of the main classes of established Galactic VHE sources, as well as of interstellar emission from cosmic-ray interactions in the Milky Way. We also perform an optimisation of the observation strategy. We use the improved sky model and observation strategy to simulate GPS data that are analysed using the methods and software tools under development for real data. We show that the GPS has the potential to increase the number of known Galactic VHE emitters by almost a factor of five. This corresponds to the detection of more than two hundred pulsar wind nebulae and a few tens of supernova remnants at average integral fluxes one order of magnitude lower than in the existing sample above 1 TeV, therefore opening the possibility to perform unprecedented population studies. The GPS also has the potential to provide new VHE detections of binary systems and pulsars, and to detect bright PeVatrons. Furthermore, the GPS will constitute a pathfinder for deeper follow-up observations of these source classes. Finally, we show that we can extract from GPS data an estimate of the contribution to diffuse emission from unresolved sources, and that there are good prospects of detecting interstellar emission and statistically distinguishing different scenarios. (Abridged)

==> text/grlb.tex <==
Gamma-ray  binaries  are  known to be variable on orbital and sometimes superorbital timescales, see, e.g.,
%\citet{Dubus13, grlbCTA19,grlbCh20}
\citet{grlbCTA19} for a review. Some of them also display spectral variability as a function of the orbital phase. Therefore for six known gamma-ray binaries and one candidate gamma-ray binary within the footprint of the GPS we introduce dedicated temporal and spectral models as detailed in table~\ref{tab:grlb}.



